Training-Free, Identity-Preserving Image Editing for Fashion Pose Alignment and Normalization

Diffusion models have recently unlocked new possibilities in editing images of real-world objects. Yet, transforming objects in non-rigid ways, such as modifying poses or applying image-based conditioning, continues to present significant challenges. Retaining the unique identity of objects during these edits is a complex task, and current techniques often fall short of delivering the precision needed for industrial settings, where consistency is non-negotiable. Additionally, adapting diffusion models demands custom training data, which is often unavailable in real-world scenarios. To address these gaps, we present FashionRepose, a novel, training-free pipeline designed to handle non-rigid pose adjustments specifically for the fashion industry. This approach combines pretrained off-the-shelf models to modify the poses of long-sleeve garments while safeguarding their identity and branding characteristics. By adopting a zero-shot methodology, FashionRepose enables near real-time edits, entirely eliminating the requirement for specialized training data. FashionRepose has been deployed for a global fashion firm, OVS, handling more than 30,000 long-sleeve garments.

==> mathematical-modelling.tex <==
\section{Methodology}

\subsection{Task Definition}

We formally define the garment pose alignment task as follows. Given an input image \(I_{in}\), representing a garment in a still-life pose, the objective is to generate an output image \(I_{out}\) with the garment repositioned to a target pose, while preserving identity, texture, and branding features.

Formally, the task is described as:

$$
I_{out} = \mathcal{T}(I_{in}, \theta_{target}),
$$

where:
- \(\mathcal{T}\) denotes the pose transformation function.
- \(\theta_{target} \in [0, 90]^\circ\) represents the target arm-torso angle.


\subsection{Pipeline Components}

The FashionRepose pipeline is articulated through distinct computational steps, each mathematically defined with inputs and outputs.


\subsubsection{Long Sleeves Detection}

This step filters relevant garment images and consists of two subcomponents: 

$$
    F_{VGG16} = \mathcal{D}_{VGG16}(I_{in}), \quad F_{VGG16} \in \{0,1\},
    $$
$$
    F_{semantic} = \mathcal{D}_{semantic}(\mathcal{F}_{caption}(I_{in})), \quad F_{semantic} \in \{0,1\},
    $$
    
where:
- \(I_{in}\) is the input still-life image,
- \(\mathcal{D}_{VGG16}\) is the VGG16-based classifier,
- \(\mathcal{F}_{caption}\) is the image captioning model,
- \(\mathcal{D}_{semantic}\) is the semantic refiner that checks textual captions.

The final outcome is obtained by combining the results:

$$
F = F_{VGG16} \land F_{semantic},
$$

where \(\land\) denotes the AND operator.


\subsubsection{Logo Suppression}

The input image \(I_{in}\) undergoes a logo suppression step to produce the logo-suppressed image \(I_{ls}\):

$$
I_{ls}, I_{logos}, M_{logos} = \mathcal{L}(I_{in}),
$$

where \(\mathcal{L}\) is the logo suppression function, \(I_{logo}\) are the extracted logos, and \(M_{logos}\) are the corresponding segmentation masks.


\subsubsection{Coarse Generation}

The Target Pose Generator module \(\mathcal{P}\) generates the target skeleton pose \(S_{pose}\) and the corresponding target pose mask \(M_{pose}\), given a specific target aperture \(\theta_{target}\):

$$
(S_{pose}, M_{pose}) = \mathcal{P}(\theta_{target}).
$$

A neck mask \(M_{neck}\) is defined as a binary 2D square matrix:

$$
(M_{neck})_{i,j} = 
\begin{cases}
1, & \text{if } i \leq 0.4 \cdot H, \\
0, & \text{otherwise},
\end{cases}
$$

where \(H\) denotes the height of the matrix, and the indices \(i\) and \(j\) denotes the pixel location within the image. The matrix has the same size as the input image \(I_{ls}\).

Embeddings \(E_{ip}\), \(E_{pose}\), and \(E_{canny}\) are subsequently obtained as follows:

- \(E_{ip}\) represents the image feature embeddings extracted from the logo-suppressed image \(I_{ls}\) using the IPAdapter  \(\mathcal{E}_{ip}\):  
$$
  E_{ip} = \mathcal{E}_{ip}(I_{ls}),
  $$
  
- \(E_{pose}\) is computed from the target skeleton pose \(S_{pose}\) by ControlNet OpenPose \(\mathcal{E}_{pose}\):

$$
E_{pose} = \mathcal{E}_{pose}(S_{pose}),
$$

- \(E_{canny}\) is computed by a ControlNet Canny model \(\mathcal{E}_{canny}\) starting from the masked canny image \(\xi\). The masked canny image is obtained via an edge detection operation \(\mathcal{X}\) applied to the target pose mask \(M_{pose}\), followed by an element-wise Hadamard product with the inverted neck mask \((1 - M_{neck})\):
  $$
  \xi = \mathcal{X}(M_{pose}) \odot (1 - M_{neck}), \quad E_{canny} = \mathcal{E}_{canny}(\xi).
  $$

The coarse representation \(I_{coarse}\) of the target pose is then generated as:

$$
I_{coarse} = \mathcal{DM}(E_{ip}, E_{pose}, E_{canny}),
$$

where \(\mathcal{DM}\) is a diffusion model serving as the coarse image generator.

\subsubsection{Conditioned Unsampling}

Latent embeddings are extracted from the logo-suppressed garment \(I_{ls}\) and the coarse pose-aligned garment \(I_{coarse}\) using the Stable Diffusion VAE encoder \(\mathcal{V}\):

$$
Z_{ls} = \mathcal{V}(I_{ls}), \quad Z_{coarse} = \mathcal{V}(I_{coarse}).
$$

A gradient-based latent blending operation produces a fused latent representation:

$$
Z_{blend} = Z_{ls} \odot Z_{gradient} + Z_{coarse} \odot (1 - Z_{gradient}),
$$

where \(Z_{gradient}\) is a gradient blending mask defined in latent space.

The Target Pose Generator \(\mathcal{P}\) produces predefined skeletons:

$$
S_{still} = \mathcal{P}(0), \quad S_{target} = \mathcal{P}(\theta_{target}).
$$

Edge maps \(\xi_{ls}\) and \(\xi_{coarse}\) are computed as:

$$
\xi_{ls} = \mathcal{X}(I_{ls}), \quad \xi_{coarse} = \mathcal{X}(I_{coarse}).
$$

ControlNet embeddings specific to each diffusion step are then computed:

- **Unsampling Embeddings**:

  $$
  \widetilde{E}_{pose}^{u} = \mathcal{E}_{pose}(S_{still}), \quad \widetilde{E}_{canny}^{u} = \mathcal{E}_{canny}(\xi_{ls}),
  $$

- **Sampling Embeddings**:

  $$
  \widetilde{E}_{pose}^{s} = \mathcal{E}_{pose}(S_{target}), \quad \widetilde{E}_{canny}^{s} = \mathcal{E}_{canny}(\xi_{coarse}).
  $$

These embeddings guide a two-stage diffusion process to obtain the refined output:

- **Unsampling Stage**:

  $$
  Z_{unsampled} = \mathcal{DM}_{unsampler}(Z_{blend}, \widetilde{E}_{pose}^{u}, \widetilde{E}_{canny}^{u}),
  $$

- **Sampling Stage**:

  $$
  I_{refined} = \mathcal{DM}(Z_{unsampled}, \widetilde{E}_{pose}^{s}, \widetilde{E}_{canny}^{s}).
  $$

where \(\mathcal{DM}_{unsampler}\) denotes the unsampling technique with a diffusion model, and \(\mathcal{DM}\) represents the standard diffusion model given an initial latents.


\subsubsection{Source-Target Shape Matching}

This step performs mask-guided shape alignment for the logo-suppressed garment and the refined garment:

$$
\overline{I}_{ls} = \mathcal{M}(I_{ls}, M_{ls}, M_{pose}),
$$

$$
\overline{I}_{refined} = \mathcal{M}(I_{refined}, M_{refined}, M_{pose}),
$$

where \(\mathcal{M}\) is the shape matching algorithm, \(M_{ls}\) and \(M_{refined}\) are the segmentation masks of the logo-suppressed garment and the refined garment, respectively, and \(M_{pose}\) is the target pose mask generated by the Target Pose Generator \(\mathcal{P}\).


\subsubsection{Garment Parts Composition}

For the garment parts composition we can define:

$$
M_{pose}^{@45} = \mathcal{P}(45),
$$
$$
I_{composed} = \mathcal{C}(\overline{I}_{refined}, \overline{I}_{ls}, M_{pose}^{@45}),
$$

where \(M_{pose}^{@45}\) is the target pose mask at a 45° angle, and \(\mathcal{P}\) is the Target Pose Generator module. The composition algorithm \(\mathcal{C}\) combines the refined garment, \(\overline{I}_{refined}\), and the logo-suppressed garment, \(\overline{I}_{ls}\), using the target pose mask \(M_{pose}^{@45}\).


\subsubsection{Logo Injection}

The composited image is upscaled:

$$
I_{composed}^{\uparrow} = \mathcal{U}_{\uparrow}(I_{composed}),
$$

Identity preservation is achieved by logo reintegration:

$$
I_{out} = \mathcal{L}^{-1}(I_{composed}^{\uparrow}, I_{logos}, M_{logos}),
$$

where \(\mathcal{L}^{-1}\) represents logo re-injection, \(I_{logos}\) are the logos extracted from \(I_{in}\) using \(\mathcal{L}\), and \(M_{logos}\) are the corresponding masks.

